Dynamic Fault Trees Analysis using an Integration of Theorem Proving and Model Checking

Dynamic fault trees (DFTs) have emerged as an important tool for capturing the dynamic behavior of system failure. These DFTs are then analyzed qualitatively and quantitatively using stochastic or algebraic methods to judge the failure characteristics of the given system in terms of the failures of its sub-components. Model checking has been recently proposed to conduct the failure analysis of systems using DFTs with the motivation to provide a rigorous failure analysis of safety-critical systems. However, model checking has not been used for the DFT qualitative analysis and the reduction algorithms used in model checking are usually not formally verified. Moreover, the analysis time grows exponentially with the increase of the number of states. These issues limit the usefulness of model checking for analyzing complex systems used in safety-critical domains, where the accuracy and completeness of analysis matters the most. To overcome these limitations, we propose a comprehensive methodology to perform the qualitative and quantitative analysis of DFTs using an integration of theorem proving and model checking based approaches. For this purpose, we formalized all the basic dynamic fault tree gates using higher-order logic based on the algebraic approach and formally verified some of the simplification properties. This formalization allows us to formally verify the equivalence between the original and reduced DFTs using a theorem prover, and conduct the qualitative analysis. We then use model checking to perform the quantitative analysis of the formally verified reduced DFT. We applied our methodology to five benchmarks and the results show that the formally verified reduced DFT was analyzed using model checking with up to six times less states and up to 133000 times faster.

==> results.tex <==
\section{Evaluation}
\label{sec:results}
In this section we presents the design of our case study aimed at assessing the effectiveness of the ATLAS scheduler. %describe the prototype we used to implement our proposed approach: to generate the log Hadoop log files, build the predictive model and to test our proposed algorithm compared to the other 3 existing implementations of Hadoop scheduler.
\subsection{Setup of the Case Study}
We instantiated 15 Hadoop machines in Amazon EMR. We set one machine to the role of master, another one to the role of secondary master (to replace the master in case of failure) and 13 machines to the role of slaves.
We selected 3 different types of machines to have heterogeneous environment which represents a real world environment hosting real and different machines.
The three types of Amazon EMR machines are \textit{m3.large}, \textit{m4.xlarge} and \textit{c4.xlarge}~\cite{AmazonInstances}. 
Details about their characteristics are listed in Table~\ref{Table:CharacteristiqueMachines}.
We choose these types of machine since they can support different workloads and they were widely used in the literature to test many systems in cloud environment. In addition, different types of Amazon EMR instance allow to have a real world cluster
where different types of machines are used.\\

\noindent We used the AnarchyApe tool described in~\cite{Faghri-Failure2012} to create different failure scenarios in Hadoop nodes such as TaskTarcker and DataNode failures, slowdown or drop in the network, loss of some job data, failure of tasks/jobs, and so on.
Specifically, we killed/suspended DataNodes/TaskTrackers; disconnected/slowed/dropped network; and randomly killed/suspended threads within DataNodes/TaskTrackers in the running executions.
To specify the amount of failures to be injected in the Hadoop clusters, we performed a quantitative analysis of failures in the public Google Traces~\cite{Mbarka15}, which contains different types of jobs (including Hadoop jobs). The public Google Traces provides data about task and job failures in real world Google clusters. %We used the results of our analysis of failures in Google traces to decide about the failure injection rates used in our case study.
We found that more than 40\% of the tasks and jobs can be failed~\cite{Mbarka15}. Therefore, in our case study,
we performed different simulations of varying the injected failure rates, with a maximum failure rate of 40\%.\\

\noindent To generate the jobs, we used the \textit{WordCount}, \textit{TeraGen} and \textit{TeraSort} examples provided by Apache, as job unit to create single or chained jobs as described in Section~\ref{dataextraction}.
The generated jobs represent different job pattern from real world applications.
These jobs have different input files (\eg{} books\footnote{http://www.gutenberg.org/wiki/Main\_Page})
that we downloaded to have large set of data to process. For each single job, we decided on the number of map and reduce tasks using information about the number of HDFS blocks in the input files. For example, we had jobs with 10 map tasks and 15 reduce tasks.
For each chained job, we decided on the number of job unit within each chain (\eg{} 3 jobs, 20 jobs), the type of used job (\eg{} \textit{WordCount}, \textit{TeraSort}) and the structure of the jobs (\eg{} sequential, parallel and mix chains).
For each type of Hadoop scheduler (\ie{} FIFO, Fair, Capacity), we generated several single and chained jobs and collected their execution logs to build the task failure prediction model required by ATLAS. %then we collect their log files to be used for the predictive models.
We built prediction models using all the classification algorithms described in Section~\ref{models} and assessed their performances following the 10-fold cross-validation approach described in Section~\ref{models}.
Also, we retrained the prediction models in the instantiated Amazon EMR machines which represent a cloud environment where drastic changes may occur because of unreliable machines. This step was performed each 10 min to make the proposed system more robust.
We implemented ATLAS using the prediction model that achieved the best performance, and compared the performance of Hadoop equipped respectively with the FIFO scheduler, the Fair scheduler, the capacity scheduler, and our proposed ATLAS scheduler integrated with these 3 existing schedulers. All the comparisons were done using the exact same jobs and data. We measured the performance each Hadoop's scheduler using the total execution times of jobs, the amount of resources used (CPU, memory, HDFS Read/Write), the numbers of finished and failed tasks, and the numbers of finished and failed jobs.

%with and without failure for the 3 implementations of Hadoop scheduler and our proposed scheduler in terms of execution time, number of failure and resources utilisation (CPU, memory, HDFS Read/Write).
\begin{table}
\caption{Amazon EC2 Instance Specifications}
\vspace{-5pt}
\centering \scriptsize
\label{Table:CharacteristiqueMachines}
\begin{tabular}{|c|c|c|c|c|}
\hline
{\bf \begin{tabular}[c]{@{}c@{}}Machine \\ Type\end{tabular}} & {\bf vCPU\textsuperscript{*}} & {\bf \begin{tabular}[c]{@{}c@{}}Memory\\ (GiB)\end{tabular}} & {\bf \begin{tabular}[c]{@{}c@{}}Storage \\ (GB)\end{tabular}} & {\bf \begin{tabular}[c]{@{}c@{}}Network \\ Performance\end{tabular}} \\ \hline
{\bf m3.large}                                                & 1          & 3.75                                                         & 4                                                             & Moderate                                                             \\ \hline
{\bf m4.xlarge}                                               & 2          & 8                                                            & EBS-Only\textsuperscript{+}                                                      & High                                                                 \\ \hline
{\bf c4.xlarge}                                               & 4          & 7.5                                                          & EBS-Only\textsuperscript{+}                                                      & High                                                                 \\ \hline
\end{tabular}
\begin{tablenotes}
      \footnotesize
      \item   \textsuperscript{*} Each vCPU is a hyperthread of an Intel Xeon core~\cite{AmazonInstances}.
      \item   \textsuperscript{+} Amazon EBS is a block-level storage volume attached to a running Amazon EC2 instance~\cite{AmazonInstances}.
   \end{tablenotes}
   \vspace{-15pt}
\end{table}

\subsection{Case Study Results}
%\vspace{-5pt}
\subsubsection{Prediction Algorithms}\label{predictionresults}
\noindent Table~\ref{Table:crossvalisationresults} summarises the performance of the six prediction models applied on data collected from the schedulers' logs. This result shows that the Random Forest algorithm achieves the best precision, recall, accuracy and error when predicting the scheduling outcome of the Map and Reduce tasks for the three studied schedulers (FIFO, Fair and Capacity).
This is because Random-Forest algorithm uses the majority voting on decision trees to generate results which makes it robust to noise, resulting usually in highly accurate predictions.
For map tasks, a Random Forest model can achieve an accuracy up to 83.7\%, a precision up to 86.4\%, a recall up to 94.3\% and an error up to 21.7\%.
The total execution time of the 10-fold cross-validation was 25.97 ms.
For reduce tasks, the Random Forest model achieved an accuracy up to 95.3\%, a precision up to 98.1\%, a recall up to 95.9\% and an error up to 16.6\%.
The total execution time of the evaluation of Random Forest for reduce tasks was 35.65 ms.
Also, we noticed that Random Forest is achieving these results in a acceptable time compared to the other algorithms (for example, the Boost algorithm can take up to 297.29 ms which can affect the performance of the scheduler).
In addition, we also found a strong correlation between the number of running/finished/failed tasks on a TaskTracker, the locality of the tasks, the number of previous finished/failed attempts of a task, and the scheduling outcome of the task. More specifically, tasks characterized by multiple past failed attempts, many concurrent tasks (running on the same TaskTracker) that experienced multiple failed attempts, have a high probability to fail in the future.
\begin{table*}[ht!]
\caption{Accuracy, Precision, Recall, Error (\%) and Time(ms) for different Algorithms: (Random 10-fold Cross-validation)}
\vspace{-5pt}
\centering \tiny
\label{Table:crossvalisationresults}
\begin{tabular}{|> {\centering\arraybackslash}p{0.8cm}|> {\centering\arraybackslash}p{1.2cm}|> {\centering\arraybackslash}p{0.3cm}|> {\centering\arraybackslash}p{0.3cm}|> {\centering\arraybackslash}p{0.3cm}|> {\centering\arraybackslash}p{0.3cm}|> {\centering\arraybackslash}p{0.6cm}|> {\centering\arraybackslash}p{0.3cm}|> {\centering\arraybackslash}p{0.3cm}|> {\centering\arraybackslash}p{0.3cm}|> {\centering\arraybackslash}p{0.3cm}|> {\centering\arraybackslash}p{0.6cm}|> {\centering\arraybackslash}p{0.3cm}|> {\centering\arraybackslash}p{0.3cm}|> {\centering\arraybackslash}p{0.3cm}|> {\centering\arraybackslash}p{0.3cm}|> {\centering\arraybackslash}p{0.6cm}|}
\hline
{\bf Task}                         & {\bf Scheduler}      & \multicolumn{5}{c|}{{\bf FIFO}}                                     & \multicolumn{5}{c|}{{\bf Fair}}                                     & \multicolumn{5}{c|}{{\bf Capacity}}                                 \\ \hline \hline
\multirow{7}{*}{{\bf Map}}    & {\bf Algo.}      & {\bf Acc.}     & {\bf Pre.}     & {\bf Rec.}     & {\bf Err.} & {\bf Time}      & {\bf Acc.}     & {\bf Pre.}     & {\bf Rec.}     & {\bf Err.}   & {\bf Time}         & {\bf Acc.}     & {\bf Pre.}     & {\bf Rec.}     & {\bf Err.} & {\bf Time}           \\ \cline{2-17}
                                   &
{\bf Tree}           & 68.6           & 85.3           & 74.3       &  31.4  & 12.34      &       92.6           & 85.2           & 62.1        &  7.4 & 9.14    &         68.7           & 85.7           & 73.4         & 31.3 & 58.18            \\ \cline{2-17}
                                   &
{\bf Boost}          & 75.9           & 86.7           & 78.5         & 24.1 & 180.51           & 65.9           & 85.6           & 73.5        &  34.1 & 199.80        &   72.5           & 85.3           & 71.3        &  27.5 & 280.56          \\ \cline{2-17}
                                   &
{\bf Glm}            & 63.5           & 87.2           & 72.4      &  36.5   & 9.43            & 67.4           & 88.6           & 65.8           & 32.6 & 13.34    &        62.1           & 83.6           & 61.8         &  37.9 & 16.01           \\ \cline{2-17}
                                   &
{\bf CTree}          & 65.9           & 87.5           & 65.2        & 34.1  & 15.61           & 62.6           & 85.2           & 69.3           & 37.4 & 16.38           & 61.8           & 79.5          &   61.2    &   38.2    & 17.53           \\ \cline{2-17}
                                   &
{\cellcolor[gray]{.8} \bf R.F.}  & {\cellcolor[gray]{.8} \bf  83.7} & {\cellcolor[gray]{.8} \bf  86.4} & {\cellcolor[gray]{.8} \bf  94.3} & {\cellcolor[gray]{.8} \bf 16.3 } & {\cellcolor[gray]{.8} \bf  23.53}  & {\cellcolor[gray]{.8} \bf  79.8} & {\cellcolor[gray]{.8} \bf  83.9} & {\cellcolor[gray]{.8} \bf 94.0} & {\cellcolor[gray]{.8} \bf 20.2 } & {\cellcolor[gray]{.8} \bf  25.91}  & {\cellcolor[gray]{.8} \bf  78.3} & {\cellcolor[gray]{.8} \bf  85.2} & {\cellcolor[gray]{.8} \bf  89.2} & {\cellcolor[gray]{.8} \bf 21.7 } & {\cellcolor[gray]{.8} \bf  25.97} \\ \cline{2-17}
                                   &
{\bf N.N.} & 65.8           & 85.8           & 79.4          & 34.2 & 61.81          & 68.7           & 86.3           & 74.1           &31.3 & 63.61           & 72.1           & 83.6           & 72.3         &27.9  & 59.71            \\ \hline  \hline
\multirow{7}{*}{{\bf Reduce}} & {\bf Algorithm}      & {\bf Acc.}     & {\bf Pre.}     & {\bf Rec.}     & {\bf Err.}  & {\bf Time}     & {\bf Acc.}     & {\bf Pre.}     & {\bf Rec.}     & {\bf Err.} & {\bf Time}      & {\bf Acc.}     & {\bf Pre.}     & {\bf Rec.}     & {\bf Err.}  & {\bf Time}     \\ \cline{2-17}
                                   &
{\bf Tree}           & 72.4           & 95.3           & 69.3           & 27.6 & 13.51           & 72.8           & 92.2           & 73.0           & 27.8& 10.23            & 63.2           & 83.4           & 68.7           &36.8 & 13.25           \\ \cline{2-17}
                                   &
{\bf Boost}          & 83.5           & 93.4           & 85.1          & 16.5 & 297.29          & 93.1           & 98.7           & 92.3         &6.9  & 269.37          & 66.8           & 91.7           & 54.7           &33.2 & 198.37         \\ \cline{2-17}
                                   &
{\bf Glm}            & 61.9           & 92.6           & 65.1          & 38.1 & 17.32         & 77.2           & 91.3           & 75.3           &22.8 & 17.39           & 68.7           & 91.9           & 71.9       &  31.3  & 19.83           \\ \cline{2-17}
                                   &
{\bf CTree}          & 79.3           & 92.6           & 81.4          & 20.7& 16.85     &       81.4           & 91.1           & 81.3 & 18.6& 16.52      &      61.7           & 91.5           & 65.1          &38.3  & 17.13          \\ \cline{2-17}
                                   &
{\cellcolor[gray]{.8} \bf R.F.}  & {\cellcolor[gray]{.8} \bf  95.3} & {\cellcolor[gray]{.8} \bf  98.1} & {\cellcolor[gray]{.8} \bf  95.9} & {\cellcolor[gray]{.8} \bf 4.7 } & {\cellcolor[gray]{.8} \bf  35.65}  & {\cellcolor[gray]{.8} \bf  92.5} & {\cellcolor[gray]{.8} \bf  97.6} & {\cellcolor[gray]{.8} \bf  92.4} & {\cellcolor[gray]{.8} \bf 7.5 } & {\cellcolor[gray]{.8} \bf  28.54}  & {\cellcolor[gray]{.8} \bf 83.4} & {\cellcolor[gray]{.8} \bf  91.5} & {\cellcolor[gray]{.8} \bf  95.6} & {\cellcolor[gray]{.8} \bf 16.6 } & {\cellcolor[gray]{.8} \bf  27.93}  \\ \cline{2-17}
                                   &
{\bf N.N.} & 74.5           & 91.5           & 75.3         &   25.5   & 89.74       & 81.5           & 97.3           & 71.6 & 18.5 & 78.61           & 74.9           & 94.1          & 83.7         & 25.1  & 85.37          \\ \hline
\end{tabular}
\vspace{-5pt}
\end{table*}

\subsubsection{Performance Evaluation of the Schedulers}
%Number of Finished of the Jobs/Map/Tasks
As stated in Section~\ref{predictionresults}, we used the Random Forest algorithm (to predict the scheduling outcome of tasks) when implementing the proposed ATLAS scheduler. %to predict the potential outcome of a task.
Figure~\ref{fig:finsihedjobs}, Figure~\ref{fig:finsihedmaptasks} and Figure~\ref{fig:finishedreducetasks} present respectively the number of finished jobs, map and reduce tasks for the three schedulers. Overall, we observe that the number of finished jobs, map and reduce tasks in ATLAS are higher in comparison to the results obtained for the FIFO, Fair, and Capacity schedulers. %were improved compared to the basic implementation of the existing implementations of Haoop schedulers as shown in Figure~\ref{fig:finsihedjobs}, Figure~\ref{fig:finsihedmaptasks} and Figure~\ref{fig:finishedreducetasks}.
This was expected since the prediction model enables the quick rescheduling of tasks that are predicted to fail.
In addition, the improvement is larger for FIFO and Fair schedulers compared to the capacity scheduler. This happens because the capacity scheduler forces the killing of any tasks consuming more memory than configured~\cite{CapacityScheduler}. 
%
The number of finished tasks is improved by up to 46\% when using ATLAS instead of the Fair scheduler (see \textit{ATLAS-Fair} in Figure~\ref{fig:finsihedmaptasks}), and the number of finished jobs increased by 27\% when using ATLAS instead of the Fair scheduler (see \textit{ATLAS-Fair} in Figure~\ref{fig:finsihedjobs}).
%Number of Failed of the Jobs/Map/Tasks
The improvement of the number of finished jobs is lower than the improvement of the number of finished tasks since a single task failure causes the whole job to fail. %ven only one failure event) because of other scheduling constraints (resources, task constraints, etc) that cause the failure of the whole job.
We also noticed that the number of failed jobs and tasks was decreased by up to 28\% for the jobs (see \textit{ATLAS-Fair} in Figure~\ref{fig:failedjobs}) and up to 39\% for the tasks (see \textit{ATLAS-Capacity} in Figure~\ref{fig:failedmaptasks}) respectively. Moreover, we also observed that when the failure of one map task causes the failure of the dependent reduce tasks belonging to the same job, ATLAS is unable to propose a better scheduling decision (because some data are lost, as explained in Figure~\ref{Figure:exampleofjobfailure}).\\

\noindent Moreover, we noticed that the number of finished single and chained jobs was improved.
% by up to 30\% and 14\%, respectively. This is by comparing the total number of finished single jobs with the launched ones (30\%) and the total number of finished chained jobs with the submitted chained jobs (14\%).  
This was expected because ATLAS enables the successful processing of the tasks composing these jobs and because of the  dependency between the jobs within the chained jobs.
In addition, the number of finished single jobs was higher than the number of finished chained jobs. This is due to the dependency between the jobs composing the chained one (\ie{} sequential ones). Also, a single job failure in the composed chain can cause the failure of the whole chained job.

\noindent \textbf{In general, we conclude that our proposed ATLAS scheduler can reduce up to 39\% of tasks failures and up to 28\% of jobs failures that are experienced by the 3 other schedulers (\ie{} FIFO, Fair, and Capacity).}
%up to 40\% because of the scheduling outcome is impacted by the dependencies between its tasks and the shared failure information.}
%Execution time of the Jobs/Tasks:
\\

\noindent Overall, the execution time of tasks and jobs is lower for ATLAS. We attribute this outcome to the fact that \textit{ATLAS} reduces the number of launched attempts and the time spent to execute the attempts.
The total execution time of jobs was decreased on average by 10 minutes (from 20 minute to 10 minute), representing a 30\% of reduction of the total execution time of these jobs (see the \textit{ATLAS-Capacity} in Figure~\ref{fig:execjobs}) and the total execution time of tasks by about 1.33 minute (from 2.33 minute to 1 minute) (see \textit{ATLAS-Capacity}: reduce task in Figure~\ref{fig:execreduce}).
For long running jobs (running for 40-50 minutes), the reduction was up to 25 minutes (representing a 54\% reduction) over the Capacity scheduler.
In this context, we should mention that there was an overhead associated with the training phase of the predictive algorithm and the communication between the JobTracker and TaskTrackers. However, this overhead was very small and is included in the execution time of ATLAS presented on Figure~\ref{fig:execjobs}, Figure~\ref{fig:execmap}, and Figure~\ref{fig:execreduce}. In fact, the reduction in the number of failures largely compensated for this overhead.

\noindent \textbf{\textit{ALTLAS} successfully reduces the overall execution times of tasks and jobs in Hadoop.} %The execution times of tasks is also improved help to avoid the long waiting time of tasks waiting in the queue until successful processing of other tasks by processing the tasks having high probability to be finished and launch speculatively many attempts (as possible in teh cluster) to increase the probability of their successful execution.}
\begin{figure*}[ht]
\minipage{0.32\textwidth}
\scriptsize
  \includegraphics[scale=0.55]{FinishedJobs.pdf}
  \caption{\scriptsize{Finished Jobs}}\label{fig:finsihedjobs}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[scale=0.55]{FinishedMapTasks.pdf}
  \caption{\scriptsize{Finished Map Tasks}}\label{fig:finsihedmaptasks}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[scale=0.55]{FinishedReduceTasks.pdf}
  \caption{\scriptsize{Finished Reduce Tasks}}\label{fig:finishedreducetasks}
\endminipage
\vspace{-5pt}
\minipage{0.32\textwidth}
  \includegraphics[scale=0.55]{FailedJobs.pdf}
  \caption{\scriptsize{Failed Jobs}}\label{fig:failedjobs}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[scale=0.55]{FailedMapTasks.pdf}
  \caption{\scriptsize{Failed Map Tasks}}\label{fig:failedmaptasks}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[scale=0.55]{FailedReduceTasks.pdf}
  \caption{\scriptsize{Failed Reduce Tasks}}\label{fig:failedreducetasks}
\endminipage
\vspace{-5pt}
\minipage{0.32\textwidth}
  \includegraphics[width=50mm,height=45mm]{ExecTimeJobs.pdf}
  \caption{\scriptsize{Jobs Exec. Time}}\label{fig:execjobs}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=50mm,height=45mm]{ExecTimeMap.pdf}
  \caption{\scriptsize{Map Exec. Time}}\label{fig:execmap}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=50mm,height=45mm]{ExecTimeReduce.pdf}
  \caption{\scriptsize{Reduce Exec. Time}}\label{fig:execreduce}
\endminipage
\end{figure*}

%Resources Utilisation
\noindent By enabling the rescheduling of potential failed tasks in advance, ATLAS reduces the total execution time of the tasks and the number of tasks and jobs failure events. Consequently, it is expected that it will reduce resource utilisations in the cluster, since it should save the amount of resources that would have been consumed by tasks failed attempts.  %should be save. the slots that would have been used by failed tasks are expected to be made available for as well.
The results presented in Table~\ref{tab:resourcesutilisation} confirms this anticipated outcome.
In fact, by quickly rescheduling tasks predicted to be failed, ATLAS can save the resources that would have been consumed by these tasks. ATLAS speculatively executes the tasks predicted to be failed on multiple nodes to increase their chance of success. Whenever one of these tasks achieves a satisfactory progress, the other speculative executions are stopped.

\noindent \textbf{Overall, the jobs and tasks executed using ATLAS scheduling policies consumed less resources than those executed using the FIFO, Fair, or Capacity schedulers (in terms of CPU, Memory, HDFS Read and Write).}

\begin{table*}[ht!]
\centering \scriptsize
\caption{Resources Utilisation of the Different Hadoop Schedulers}
\vspace{-5pt}
\label{tab:resourcesutilisation}
\begin{tabular}{|p{1.2cm}|p{4cm}|p{0.9cm}|p{0.9cm}|p{0.9cm}|p{0.9cm}|p{0.9cm}|p{0.9cm}|}
\hline
\multirow{3}{*}{{\bf Job/Task}} & \multirow{2}{*}{{\bf Scheduler}} & \multicolumn{2}{c|}{{\bf FIFO}} & \multicolumn{2}{c|}{{\bf Fair}} & \multicolumn{2}{c|}{{\bf Capacity}} \\ \cline{3-8}
                                &                                  & {\bf Basic}    & {\bf ATLAS}    & {\bf Basic}    & {\bf ATLAS}    & {\bf Basic}       & {\bf ATLAS}     \\ \cline{2-8}
                                & {\bf Resource}                   & {\bf Avg.}     & {\bf Avg.}     & {\bf Avg.}     & {\bf Avg.}     & {\bf Avg.}        & {\bf Avg.}      \\ \hline\hline
\multirow{4}{*}{{\bf Job}}      & {\bf CPU (ms)}                        & 11495           & 8415           & 12647           & 9538           & 14475             & 10784            \\ \cline{2-8}
                                & {\bf Memory ($10^{5}$ bytes}                     & 7479     & 4530     & 7741     & 3647  & 9463        & 5486      \\ \cline{2-8}
                                & {\bf HDFS Read ($10^{3}$ bytes)}                  & 9930     & 7431     & 10968     & 8762  & 12463       & 8360      \\ \cline{2-8}
                                & {\bf HDFS Write ($10^{3}$ bytes)}                 & 8583     & 5985     & 9784     & 6202     & 10285        & 7420     \\ \hline\hline
\multirow{4}{*}{{\bf Task}}     & {\bf CPU (ms)}                        & 3855           & 2520           & 4033           & 2184           & 4170              & 2851            \\ \cline{2-8}
                                & {\bf Memory ($10^{5}$ bytes}                     & 1412     & 1058      & 2496     & 1741     & 2638        & 2115     \\ \cline{2-8}
                                & {\bf HDFS Read ($10^{5}$ bytes)}                  & 1638     & 1215     & 1894     & 1428     & 7426        & 4541      \\ \cline{2-8}
                                & {\bf HDFS Write ($10^{5}$ bytes)}                 & 1774     & 1385     & 3643     & 2429  & 5052         & 3715      \\ \hline
\end{tabular}
\vspace{-5pt}
\end{table*}



